Data Drift Monitoring for Log Anomaly Detection Pipelines

Logs enable the monitoring of infrastructure status and the performance of associated applications. Logs are also invaluable for diagnosing the root causes of any problems that may arise. Log Anomaly Detection (LAD) pipelines automate the detection of anomalies in logs, providing assistance to site reliability engineers (SREs) in system diagnosis. Log patterns change over time, necessitating updates to the LAD model defining the `normal' log activity profile. In this paper, we introduce a Bayes Factor-based drift detection method that identifies when intervention, retraining, and updating of the LAD model are required with human involvement. We illustrate our method using sequences of log activity, both from unaltered data, and simulated activity with controlled levels of anomaly contamination, based on real collected log data.

==> multinomial_assumptions.tex <==
\section{Multinomial fitting
\label{sec:multinomial_fitting}
}

In Section~\ref{ssec:multinomial} we note the use of the multinomial distribution $\mn$ to model the count vectors $\boldsymbol{C}$ of template matches.  Table~\ref{tab:simulation_summaries} shows that the FPR is in fact not typically controlled at the expected level $\alpha=0.05$ across the applications.  Here, we examine the multinomial distribution assumption.  Letting $C_N$ and $C_A$ be the collected count vectors for a particular application for years 2020 and 2022, respectively. 
Letting $\tilde{\boldsymbol{C}}=E(\boldsymbol{C})$, and $\tilde{C}_N=\{
\tilde{\boldsymbol{C}}_i^N,\colon\:i=1,\dots,|C_N|\}$,  with $\tilde{C}_A$ being defined similarly, be the set of these count vectors normalized to sum 1.  Recall that $\boldsymbol{P}_N$ and $\boldsymbol{P}_A$ are the two samples' elementwise mean vectors (Section~\ref{ssec:cv_drift_simulation}).

By using the normalized $\tilde{C}_N$ and $\tilde{C}_A$ in our simulations, we essentially view them as distributed $\mn(
\boldsymbol{P}_N,1)$ and $\mn(
\boldsymbol{P}_A,1)$, even though multinomials must be integer-valued vectors. A multinomial distributed vector $\boldsymbol{X}\sim\mn(\boldsymbol{P},n)$ has elementwise standard deviations $SD(\boldsymbol{X}[i])=\sqrt(n\boldsymbol{P}[i](1-\boldsymbol{P}[i])}$.  We can therefore compare, say, the observed sample $SD(\{\tilde{\boldsymbol{C}}_i^N\}_{i=1}^{|C_N|})$



==> old/experiments_old.tex <==
\section{Experiments}
\label{sec:experiments}

We run the training pipeline by generating templates on the 2020 data. The count vectors from 2020 data do not show any drift detected. Since the Bayes Factor considers cumulative data, it is interesting to see the effect of inference on gradual drift introduction compared to sudden drift.

The log data we used for our experiments was collected using a log aggregator, which aggregates logs from different applications (micro-services) within a certain deployment. We found 6 applications that were common to both 2020 and 2022 data, viz., DLG, MTR, NLU, MMR, STR< STRS (actual names masked for confidentiality). These applications had a distinct number of templates as well as the sum of count vectors.

We fit the Bayesian model on the 2020 log distribution and inject the 2022 logs for drift detection. 
We compare the results from Bayes Drift Detection with Logistic Regression and KL Divergence models.

\subsection{Bayes Factor}

We form a simulated dataset that contains the 1100-count vectors using Block contamination. 
The contamination factor $\pi_t$ is simulated from 0 to 1 with increments of 0.1.
The count vectors from 2020 data form our $H_0$ whereas the count vectors from 2022 data are our $H_{100}$. Thus, we gradually shift from non-drifted logs to drifted logs over time with minor increments. 
This can also be thought of as inducing an increasing number of unknown logs.
Thus, according to our convention, logs from $H_0 \dots H_{30}$ are considered non-drifted, i.e., from count vectors in time $[0-300]$ in Fig \ref{fig: drift with spikes}
We plot the Bayes Factor values vs each count vector (Fig \ref{fig: drift with spikes}) and understand the changes in its values as the type of ingested logs changes. During the simulations, we observed that if we continuously ingest non-drifted logs, the log-Bayes Factor remains near-constant with minor variations in the range of $\pm 0.01$. This can be seen for the count vector for windows 0-300.
As we start inducing drifted count vectors we see some spikes in the Bayes Factor values. We monitor these spikes and observe that as the drift increases, the frequency of spikes increases as there are frequent changes in the Bayes Factor values.
% \subsection{Comparison with KL Divergence and Logistic Regression}

\subsection{Fitting the distribution}
We simulate a training dataset to set the hyper-parameters of scaling and the initial value of alpha. This helps in determining the optimal parameters to detect the drift earlier. These parameters determine the delay in detecting the drift. 
We also ran the training and testing loop on data from the Quote of the Day simulated (QoTD) application. We observed that the Bayes Factor drops to a lower value ($10^{-50}$) and then increases when the drifted count vectors are added during inference. The spike detection algorithm is agnostic to the actual Bayes Factor values. 
\subsection{Effect of Normalization and Scaling}
By definition of our Bayes Factor
Observations:
\begin{itemize}
    \item The log(BF) should always be non-decreasing for the continuous input of count vectors
    \item The BF always has a higher value as the drift increases. If the Bayes Factor is not increasing over time it is likely that the initialization is incorrect.
    \item No other parameter from the simulation should interfere with the output of the scaling factor. 
    
\end{itemize}
\textit{}

==> results.tex <==
\section{Results on deployed data}
\label{sec:results}
    
\begin{tabular}{|c|c|c|}
\hline
Application Name & Accuracy & False Positive Rate \\
\hline
nlu & 97\% & 0.0 \\
dialog & 83\% & 0.0 \\
master& 96\% & 0.0 \\
mm-runtime & 91\% & 0.06 \\
store & 90\% & 0.0 \\
store-sync & 92\% & 0.0 \\
\hline
\end{tabular}


Change point detection

\subsection{Drift vs Anomaly}

\subsection{Scaling down factor $\propto$ time to detect drift}

